Sound-skwatter (Did You Mean: Sound-squatter?) AI-powered Generator for Phishing Prevention

Sound-squatting is a phishing attack that tricks users into malicious resources by exploiting similarities in the pronunciation of words. Proactive defense against sound-squatting candidates is complex, and existing solutions rely on manually curated lists of homophones. We here introduce Sound-skwatter, a multi-language AI-based system that generates sound-squatting candidates for proactive defense. Sound-skwatter relies on an innovative multi-modal combination of Transformers Networks and acoustic models to learn sound similarities. We show that Sound-skwatter can automatically list known homophones and thousands of high-quality candidates. In addition, it covers cross-language sound-squatting, i.e., when the reader and the listener speak different languages, supporting any combination of languages. We apply Sound-skwatter to network-centric phishing via squatted domain names. We find ~ 10% of the generated domains exist in the wild, the vast majority unknown to protection solutions. Next, we show attacks on the PyPI package manager, where ~ 17% of the popular packages have at least one existing candidate. We believe Sound-skwatter is a crucial asset to mitigate the sound-squatting phenomenon proactively on the Internet. To increase its impact, we publish an online demo and release our models and code as open source.

==> Makefile <==
DOC=main

all:
	pdflatex -shell-escape $(DOC)
	bibtex   $(DOC)
	pdflatex -shell-escape $(DOC)
	pdflatex -shell-escape $(DOC)

clean:
	find . -name '*~' -exec rm -f {} \;
	find . -name '*.aux' -exec rm -f {} \;
	rm -f texput.log $(DOC).log $(DOC).ps $(DOC).toc $(DOC).lo* $(DOC).bbl $(DOC).blg $(DOC).dvi $(DOC).out $(DOC).synctex.gz

# markup:
# 	latexdiff -f FLOATSAFE -c latexdiff_conf.txt --preamble=latexdiff_preamble.tex \
# 		--flatten tnsm_1st/main.tex main.tex > diff2.tex
# 	./diff/cleanup.py -f diff2.tex > diff.tex
# 	pdflatex --synctex=1 -shell-escape diff
# 	pdflatex --synctex=1 -shell-escape diff
# final:
# 	pdflatex --synctex=1 -shell-escape diff
# 	pdflatex --synctex=1 -shell-escape diff

